Janus: Efficient and Accurate Dual-radio Social Contact Detection

Determining when two individuals are within close distance is key to contain a pandemic, e.g., to alert individuals in real-time and trace their social contacts. Common approaches rely on either Bluetooth Low Energy (BLE) or ultra-wideband (UWB) radios, that nonetheless strike opposite tradeoffs for energy efficiency vs. accuracy of distance estimates. Janus reconciles these dimensions with a dual-radio protocol enabling efficient and accurate social contact detection. Measurements show that Janus achieves weeks to months of autonomous operation, depending on the configuration. Several large-scale campaigns in real-world contexts confirm its reliability and practical usefulness in enabling insightful analysis of contact data.

==> bios.tex <==

\section*{Biographies}

\begin{IEEEbiographynophoto}{Timofei Istomin}
  is a postdoctoral researcher at University of Trento,
  focusing on low-power wireless communication protocols and
  localization techniques for networked embedded systems and the
  Internet of Things. He received his PhD degree from the same
  university in 2017.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Elia Leoni}
  is a PhD student at Fondazione Bruno Kessler in Trento.  He received
  his MS degree in Electronics and Telecommunications Engineering from
  the University of Bologna in 2019. His research centers on wireless
  sensor networks and the Internet of Things, focusing on protocols
  and communication.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Davide Molteni}
  is a Research Assistant at the University of Trento. After
  his MS in Telecommunication Engineering in 2010 on wireless sensor
  networks applied to wildlife, he works in the same general field,
  focusing on firmware development, hardware integration, and in-field
  deployments.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Amy L. Murphy}
  is a researcher at Fondazione Bruno Kessler in Trento. Her
  research focuses on applied research for smart cities from the
  perspective of software engineering, distributed computing, and
  low-power wireless networks.  The driving theme in her work is
  enabling reliable applications for dynamic environments with
  attention to the wireless communication protocols necessary to
  support complex interactions among distributed devices.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Gian Pietro Picco}
  is a professor at the University of Trento. His research spans the
  fields of software engineering, middleware, and networking, focusing
  on low-power wireless networking for cyber-physical systems and the
  Internet of Things. He is the recipient of several awards, an
  associate editor for ACM Trans. on Sensor Networks (TOSN), and
  co-Editor-in-Chief of ACM.~Trans. on Internet of Things (TIOT).
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Maurizio Griva}
  is a senior manager, head of R\&D projects of the IoT Solutions
  division at Concept Reply, a company belonging to the Reply
  group. He has more than 20 years of industry experience in
  electronic product design, embedded software and wireless wearable
  device development. 
\end{IEEEbiographynophoto}

\vfill

